Learning Models from Data with Measurement Error: Tackling Underreporting

Measurement error in observational datasets can lead to systematic bias in inferences based on these datasets. As studies based on observational data are increasingly used to inform decisions with real-world impact, it is critical that we develop a robust set of techniques for analyzing and adjusting for these biases. In this paper we present a method for estimating the distribution of an outcome given a binary exposure that is subject to underreporting. Our method is based on a missing data view of the measurement error problem, where the true exposure is treated as a latent variable that is marginalized out of a joint model. We prove three different conditions under which the outcome distribution can still be identified from data containing only error-prone observations of the exposure. We demonstrate this method on synthetic data and analyze its sensitivity to near violations of the identifiability conditions. Finally, we use this method to estimate the effects of maternal smoking and opioid use during pregnancy on childhood obesity, two import problems from public health. Using the proposed method, we estimate these effects using only subject-reported drug use data and substantially refine the range of estimates generated by a sensitivity analysis-based approach. Further, the estimates produced by our method are consistent with existing literature on both the effects of maternal smoking and the rate at which subjects underreport smoking.

==> misclassification.tex <==
Assume that we are interested in estimating $p(Y|A,X)$, the distribution of a binary outcome $Y\in\{0,1\}$ given a binary exposure binary exposure $A \in \{0,1\}$ and a set of known confounders $X\in\mathbb{R}^d$\footnote{Under the assumptions of consistency, positivity, and conditional exchangeability, this distribution could be used to estimate the causal effect of $A$ on $Y$ \ref{hernan2018causal}.}; however, rather than observing $A$, we observe an error-prone version $\tilde{A} \in \{0,1\}$. For example, $A$ might represent true drug use while $\tilde{A}$ represents subject-reported drug use. For reasonably high-dimensional $X$, this is typically done using a parametric outcome model which, if we were able to observe $A$, could be estimated directly from data. Instead, our goal is to estimate $p(Y|A,X)$ from a dataset $\mathcal{D}=\{(x_i,\tilde{a}_i,y_y)\}_{i=1}^N$ consisting only of the outcome, covariates, and error-prone exposure observation. In order to make this possible it is necessary to make some modeling assumptions.

% Using notation from the potential outcomes literature, we are interested in estimating $\mathbf{E}[Y^a]$ where $Y^a$ is the potential outcome under exposure $a$ \cite{hernan2018causal}. Under the assumptions of consistency, positivity, and conditional exchangeability, $\mathbf{E}[Y^a]$ can be calculated from observable quantities as:
% %
% \begin{align*}
% 	\mathbf{E}[Y^a] &= \mathbf{E}[\mathbf{E}[Y|A=a,X]]\\ &\approx \frac{1}{N} \sum_i \mathbf{E}[Y|A=a,X=x_i]
% \end{align*}
% %
% where the outer expectation is over $X$ and the inner expectation is over $Y$. Even without the conditional exchangeability assumption, the quantity $\mathbf{E}[\mathbf{E}[Y|A=a,X]]$ may be of interest for measuring (potentially confounded) associations between $A$ and $Y$. In order to estimate this quantity, we must first estimate $\mathbf{E}[Y|A,X]$, which for binary outcomes is equivalent to estimating $p(Y|A,X)$. For reasonably high-dimensional $X$, this is typically done using a parametric outcome model which, if we were able to observe $A$, could be estimated directly from data. Instead, our goal is to estimate $p(Y|A,X)$ from a dataset $\mathcal{D}=\{(x_i,\tilde{a}_i,y_y)\}_{i=1}^N$ consisting only of the outcome, covariates, and error-prone exposure observation. In order to make this possible it is necessary to make some modeling assumptions.
